Estimating the Robustness of Classification Models by the Structure of the Learned Feature-Space

Over the last decade, the development of deep image classification networks has mostly been driven by the search for the best performance in terms of classification accuracy on standardized benchmarks like ImageNet. More recently, this focus has been expanded by the notion of model robustness, \ie the generalization abilities of models towards previously unseen changes in the data distribution. While new benchmarks, like ImageNet-C, have been introduced to measure robustness properties, we argue that fixed testsets are only able to capture a small portion of possible data variations and are thus limited and prone to generate new overfitted solutions. To overcome these drawbacks, we suggest to estimate the robustness of a model directly from the structure of its learned feature-space. We introduce robustness indicators which are obtained via unsupervised clustering of latent representations from a trained classifier and show very high correlations to the model performance on corrupted test data.

==> old_4_2_latent_space.tex <==
\subsection{Latent Space Clustering with K-means and Multicuts}
\label{subsec:latentspace}

We compare two clustering methods: \textit{k-means} on the left and \textit{multicuts}.
The extracted feature vectors were used to evaluate different models and we report the cluster accuracy and purity score.
An overview is provided in Table~\ref{table:corrupt}.
The hyperparameter $k$ on \textit{k-means} was set to $k=1000$ and the threshold for \textit{multicuts} was estimated empirically.  We provide details in the Supplementary Materials.
In all cases, the clustering accuracy is lower than its original classification performance.
On the \textit{nasnetamobile} and \textit{inceptionresnetv2} latent spaces, \textit{multicuts} perform slightly better than \textit{k-means}. On other models, \textit{multicuts} show lower clustering accuracies. It can be observed that the multicut clustering accuracy does not reflect a model's classification accuracy. However, this is to be expected as the multicut problem is not aware of the number of classes in the original classification problem.

==> z_4_2_dim_reduction.tex <==
\subsection{Dimensionality Reduction using PCA}
\label{subsec:dim_red}

\begin{table}[t]
    \caption{Principal component analysis (PCA) on features: AlexNet with the largest feature size has also the highest compression. In bold: highest number of principal components (e.g. "least reduction of features") with highest clustering accuracy (ACC).}
    \label{table:pca_variance}
    \vskip -0.12in
    \begin{center}
        \begin{small}
            \begin{sc}
                \begin{tabular}{l r r r | r | r }
                \toprule
                Model & Feat. & 75\% & 80\% & Top1\% & ACC \\
                \midrule
                alexnet & 4.096 & 29 & 36 & 56.4 & 14.5  \\
                namobile & 1.056 & 118 & 143 & 74.1 & 43.1 \\
                densenet121 & 1.024 & 161 & 196 & 74.6 & 48.9 \\
                resnet50 & 2.048 & 121 & 146 & 76.0 & 54.9 \\
                IncResNv2 & 1.536 & \textbf{254} & \textbf{304} & 80.2 & \textbf{70.2} \\
                polynet & 2.048 & 194 & 244 & 81.0 & 67.7 \\
                \midrule
                Deit-tiny & 192 & 113 & 125 & 74.5 & 56.4 \\
                Deit-small & 384 & \textbf{222} & \textbf{247} & 81.2 & \textbf{68.8} \\
                \bottomrule
                \end{tabular}
            \end{sc}
        \end{small}
    \end{center}
    \vskip -0.25in
\end{table}

While the overlap $\Delta$ may provide a good estimate regarding the quality of the features, the dimension size of the feature vector varies across different architectures. As we argue in section \ref{lb:PCA}, we want to investigate the relationship between the expressiveness of the learned features and their required number of dimensions.
%If models show similar performance in classification task, their features should also be equally discriminative and expressive.
%Furthermore, it should be possible to represent features with equal size of dimensions.
%Motivated by this, we reduce the features using principal component analysis (PCA), which has been done on CNN-features in the past~\cite{babenko2014neural, cao2018image}.

In Table~\ref{table:pca_variance}, we report the dimension size of the feature, which first reaches the cumulative sum of explained variance ratio.
This is the ratio between the eigenvalue of a particular principal component and the sum of eigenvalues.
For instance, \textit{alexnet} requires 7 additional principal components to reach from 75\% to 80\% of cumulative explained ratio. 
Though it has the lowest top 1\% classification performance with the highest reduction (from 4096 to 29 at 75\%), other models seem to have a range of principal components between \numrange[range-phrase = --]{100}{200}.
The highest number of principal components at 75\% is observed for \textit{InceptionResnetv2} (e.g. the least compression) and at the same time highest clustering accuracy.
This suggests an additional indicator for the separability of the features.
Additionally, we ran an evaluation on corrupted images for all severity levels. 
Figure~\ref{fig:pca_robust} shows a strong correlation between the principal components at 75\% against the ratio between \textit{kmeans} clustering accuracy, clean and corruption on 5 severity levels, and classification performance.
The lower the ratio between clustering and classification performance the less principal components are required.

\begin{figure}[H]
    \vskip -0.2in
    \begin{center}
        \centerline{\includegraphics[width=1.1\columnwidth]{images/4_2_pca_robust.pdf}}
        \caption{Principal Components vs. Ratio between the classification accuracy on corrupted features with its baseline.
        A strong correlation ($R^2=0.78$) is observed.}
        \label{fig:pca_robust}
    \end{center}
    \vskip -0.4in
\end{figure}

\textbf{Clustering.} We apply \textit{kmeans} clustering on the features before and after PCA with $k$ (number of clusters) set to $k=1000$.
The optimal number of components used for the reduction is provided in supplementary materials.
We report the clustering performance in Figure~\ref{fig:pca_runtime}.
\textit{InceptionResnetv2} and the transformer model \textit{Deit\_s} achieve the highest clustering accuracy of 70.2\% and 68.8\%, respectively.
Although reducing the dimension size of the feature vectors with PCA has almost little to no effect on the final results of \textit{kmeans}, the number on Table~\ref{table:pca_variance} provides another hint regarding the quality of features: both models have the highest number of principal components at 75\% and 80\% and also perform best on the cluster task.

\begin{figure}[H]
    \vskip 0.1in
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{images/4_2_acc_runtime.pdf}}
        \caption{\textit{kmeans} clustering accuracy on feature vectors before and after PCA on ImageNet test dataset: runtime decreases significantly, while little to no effect on clustering performance.}
        \label{fig:pca_runtime}
    \end{center}
    \vskip -0.4in
\end{figure}

==> z_4_4_multicut.tex <==
\noindent\textbf{Decision Boundary on Multicuts Clustering}
%\label{subsec:multicut_clustering}
The threshold for \textit{multicuts} clustering is a crucial hyperparameter: for our experiment, this decision boundary is estimated empirically on a small subset of the dataset.
For instance, if the threshold is set too high, less clusters are produced.
Choosing a lower threshold results in high number of clusters.
Figure~\ref{fig:multicut_threshold} shows the relationship between the choice of threshold and the cluster performance.
In this particular experiment, we first obtain the optimal threshold empirically and we set the range small in order to emphasize the sensitivity of \textit{multicuts} regarding the threshold and the number of clusters (note that the right y-axis indicates number of clusters in thousands).
Despite the cluster accuracy (blue line) remaining stable within the selected threshold ranges, which suggests correctly grouped images with high confidence, the number of clusters varies significantly (red line).
Selecting a decision boundary results in less clusters.
When choosing a low threshold, a rise in purity score is observed, which mostly clusters with a single image contributes to it (trivial case).

Surprisingly, \textit{NasnetAmobile} achieves better results compared to \textit{Densenet121},  \textit{ResNet50} or \textit{Deit\_t}, despite having lower cluster performance on \textit{kmeans}.
Additionally, \textit{multicuts} is able to cluster the data correctly, despite having a large overlap in intra- and inter-class distances (refer to Figure~\ref{fig:intra_inter_dist}).
On the other hand, the high number of principal components on \textit{NasnetAmobile} required to reach 75\% of cumulative explained variances (see Table~\ref{table:pca_variance}) indicates the expressiveness of the features.

\begin{figure*}[h]
    \vskip 0.2in
    \begin{center}
        \centerline{\includegraphics[width=1.0\textwidth]{images/4_4_mc.pdf}}
        \caption{Clustering performance of \textit{multicuts} on different model architectures for different thresholds: the stacked bar represents the purity score, grouped by cluster with size of 1 (dark orange) and clusters with size larger than 1 (light orange). The blue line represents the cluster accuracy (ACC) while the red line the number to total unique clusters. This experiment was conducted on a subset of the test dataset.}
        \label{fig:multicut_threshold}
    \end{center}
    \vskip 0.2in
\end{figure*}
